The Design, Construction, Operation and Performance of the Belle II Silicon Vertex Detector

The Silicon Vertex Detector of Belle II is a state-of-the-art tracking and vertexing system based on double-sided silicon strip sensors, designed and fabricated by a large international collaboration in the period 2012--2018. Since 2019 it has been in operation providing high quality data with a small number of defective channels (<1%), a large hit-finding efficiency (>99%), a good signal-to-noise ratio (well in excess of 10 for all sensor configurations and tracks). Together with the good control over the alignment, these are all essential factors to achieve good tracking reconstruction and physics performance. In this extended paper we try to document all the aspects of the SVD challenges and achievements, in the spirit of providing information to the broader community and help the development of high quality detector systems, which are fundamental tools to carry out physics research.

==> svd-sym.tex <==
%%%%%   Standard symbols for use in Belle II notes and papers. 
%%%%%
%%%%%	C. Hearty	21-Oct-2014		Based on babarsym.tex; authored by D. Hitlin, D. MacFarlane, P. Dauncey, and R. Waldi
%%%%%

%% Can be updatd with SVD-specific symbols

\RequirePackage{xspace}

%%%%%%%%%%%%%%%%%%%% THE NAME OF THE COLLABORATION %%%%
\newcommand{\belletwo}{Belle~II}
%
% Note that latex macros cannot contain numbers, only letters !
%
\newcommand{\phaseone}{Phase~1}
\newcommand{\phasetwo}{Phase~2}
\newcommand{\phasethree}{Phase~3}
\newcommand{\COtwo}{CO$_2$}
\newcommand{\vsep}{$\rm{V}_{\rm SEP}$}
\newcommand{\airex}{AIREX\textsuperscript{\textregistered} }
\newcommand{\apv}{APV25}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%   LEPTONS   %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\let\emi\en
\def\electron   {\ensuremath{e}\xspace}
\def\en         {\ensuremath{e^-}\xspace}   % electron negative (\em is taken)
\def\ep         {\ensuremath{e^+}\xspace}
\def\epm        {\ensuremath{e^\pm}\xspace} 
\def\epem       {\ensuremath{e^+e^-}\xspace}
\def\ee         {\ensuremath{e^-e^-}\xspace}

\def\qqbar       {\ensuremath{q\bar{q}}\xspace}

\def\mmu        {\ensuremath{\mu}\xspace}
\def\mup        {\ensuremath{\mu^+}\xspace}
\def\mun        {\ensuremath{\mu^-}\xspace} % muon negative (\mum is taken)
\def\mumu       {\ensuremath{\mu^+\mu^-}\xspace}
\def\mtau       {\ensuremath{\tau}\xspace}

\def\taup       {\ensuremath{\tau^+}\xspace}
\def\taum       {\ensuremath{\tau^-}\xspace}
\def\tautau     {\ensuremath{\tau^+\tau^-}\xspace}

\def\ellm       {\ensuremath{\ell^-}\xspace}
\def\ellp       {\ensuremath{\ell^+}\xspace}
\def\ellell     {\ensuremath{\ell^+ \ell^-}\xspace}

\def\nub        {\ensuremath{\overline{\nu}}\xspace}
\def\nunub      {\ensuremath{\nu{\overline{\nu}}}\xspace}
\def\nub        {\ensuremath{\overline{\nu}}\xspace}
\def\nunub      {\ensuremath{\nu{\overline{\nu}}}\xspace}
\def\nue        {\ensuremath{\nu_e}\xspace}
\def\nueb       {\ensuremath{\nub_e}\xspace}
\def\nuenueb    {\ensuremath{\nue\nueb}\xspace}
%\def\num        {\ensuremath{\nu_\mu}\xspace}
%\def\numb       {\ensuremath{\nub_\mu}\xspace}
%\def\numnumb    {\ensuremath{\num\numb}\xspace}
\def\nut        {\ensuremath{\nu_\tau}\xspace}
\def\nutb       {\ensuremath{\nub_\tau}\xspace}
\def\nutnutb    {\ensuremath{\nut\nutb}\xspace}
\def\nul        {\ensuremath{\nu_\ell}\xspace}
\def\nulb       {\ensuremath{\nub_\ell}\xspace}
\def\nulnulb    {\ensuremath{\nul\nulb}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%  PHOTONS  %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\g     {\ensuremath{\gamma}\xspace}
\def\gaga  {\ensuremath{\gamma\gamma}\xspace}  %% changed from \gg, which is >>
\def\ggstar{\ensuremath{\gamma\gamma^*}\xspace}

\def\ega    {\ensuremath{e\gamma}\xspace}
\def\game   {\ensuremath{\gamma e^-}\xspace}
\def\epemg  {\ensuremath{e^+e^-\gamma}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%  Other GAUGE BOSONS  %%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\H      {\ensuremath{H^0}\xspace}
\def\Hp     {\ensuremath{H^+}\xspace}
\def\Hm     {\ensuremath{H^-}\xspace}
\def\Hpm    {\ensuremath{H^\pm}\xspace}
\def\W      {\ensuremath{W}\xspace}
\def\Wp     {\ensuremath{W^+}\xspace}
\def\Wm     {\ensuremath{W^-}\xspace}
\def\Wpm    {\ensuremath{W^\pm}\xspace}
\def\Z      {\ensuremath{Z^0}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%   QUARKS   %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\q     {\ensuremath{q}\xspace}
\def\qbar  {\ensuremath{\overline q}\xspace}
\def\qqbar {\ensuremath{q\overline q}\xspace}
\def\u     {\ensuremath{u}\xspace}
\def\ubar  {\ensuremath{\overline u}\xspace}
\def\uubar {\ensuremath{u\overline u}\xspace}
\def\d     {\ensuremath{d}\xspace}
\def\dbar  {\ensuremath{\overline d}\xspace}
\def\ddbar {\ensuremath{d\overline d}\xspace}
\def\s     {\ensuremath{s}\xspace}
\def\sbar  {\ensuremath{\overline s}\xspace}
\def\ssbar {\ensuremath{s\overline s}\xspace}
\def\c     {\ensuremath{c}\xspace}
\def\cbar  {\ensuremath{\overline c}\xspace}
\def\ccbar {\ensuremath{c\overline c}\xspace}
\def\b     {\ensuremath{b}\xspace}
\def\bbar  {\ensuremath{\overline b}\xspace}
\def\bbbar {\ensuremath{b\overline b}\xspace}
\def\t     {\ensuremath{t}\xspace}
\def\tbar  {\ensuremath{\overline t}\xspace}
\def\tbar  {\ensuremath{\overline t}\xspace}
\def\ttbar {\ensuremath{t\overline t}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% LIGHT MESONS  %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\piz   {\ensuremath{\pi^0}\xspace}
\def\pizs  {\ensuremath{\pi^0\mbox\,\rm{s}}\xspace}
\def\ppz   {\ensuremath{\pi^0\pi^0}\xspace}
\def\pip   {\ensuremath{\pi^+}\xspace}
\def\pim   {\ensuremath{\pi^-}\xspace}
\def\pipi  {\ensuremath{\pi^+\pi^-}\xspace}
\def\pipm  {\ensuremath{\pi^\pm}\xspace}
\def\pimp  {\ensuremath{\pi^\mp}\xspace}
\def\pis   {\ensuremath{\pi_{\rm s}}\xspace}
\def\pips   {\ensuremath{\pi^+_{\rm s}}\xspace}

\def\kaon  {\ensuremath{K}\xspace}
%%% do NOT use ensuremath here
\def\Kbar  {\kern 0.2em\overline{\kern -0.2em K}{}\xspace}
\def\Kb    {\ensuremath{\Kbar}\xspace}
\def\Kz    {\ensuremath{K^0}\xspace}
\def\Kzb   {\ensuremath{\Kbar^0}\xspace}
\def\KzKzb {\ensuremath{\Kz \kern -0.16em \Kzb}\xspace}
\def\Kp    {\ensuremath{K^+}\xspace}
\def\Km    {\ensuremath{K^-}\xspace}
\def\Kpm   {\ensuremath{K^\pm}\xspace}
\def\Kmp   {\ensuremath{K^\mp}\xspace}
\def\KpKm  {\ensuremath{\Kp \kern -0.16em \Km}\xspace}
\def\KS    {\ensuremath{K^0_{\scriptscriptstyle S}}\xspace} 
\def\KL    {\ensuremath{K^0_{\scriptscriptstyle L}}\xspace} 
\def\Kstarz  {\ensuremath{K^{*0}}\xspace}
\def\Kstarzb {\ensuremath{\Kbar^{*0}}\xspace}
\def\Kstar   {\ensuremath{K^*}\xspace}
\def\Kstarb  {\ensuremath{\Kbar^*}\xspace}
\def\Kstarp  {\ensuremath{K^{*+}}\xspace}
\def\Kstarm  {\ensuremath{K^{*-}}\xspace}
\def\Kstarpm {\ensuremath{K^{*\pm}}\xspace}
\def\Kstarmp {\ensuremath{K^{*\mp}}\xspace}

\newcommand{\etapr}{\ensuremath{\eta^{\prime}}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% HEAVY MESONS  %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% do NOT use ensuremath here
\def\Dbar    {\kern 0.2em\overline{\kern -0.2em D}{}\xspace}
\def\Db      {\ensuremath{\Dbar}\xspace}
\def\Dz      {\ensuremath{D^0}\xspace}
\def\Dzb     {\ensuremath{\Dbar^0}\xspace}
\def\DzDzb   {\ensuremath{\Dz {\kern -0.16em \Dzb}}\xspace}
\def\Dp      {\ensuremath{D^+}\xspace}
\def\Dm      {\ensuremath{D^-}\xspace}
\def\Dpm     {\ensuremath{D^\pm}\xspace}
\def\Dmp     {\ensuremath{D^\mp}\xspace}
\def\DpDm    {\ensuremath{\Dp {\kern -0.16em \Dm}}\xspace}
\def\Dstar   {\ensuremath{D^*}\xspace}
\def\Dstarb  {\ensuremath{\Dbar^*}\xspace}
\def\Dstarz  {\ensuremath{D^{*0}}\xspace}
\def\Dstarzb {\ensuremath{\Dbar^{*0}}\xspace}
\def\Dstarp  {\ensuremath{D^{*+}}\xspace}
\def\Dstarm  {\ensuremath{D^{*-}}\xspace}
\def\Dstarpm {\ensuremath{D^{*\pm}}\xspace}
\def\Dstarmp {\ensuremath{D^{*\mp}}\xspace}
\def\Ds      {\ensuremath{D^+_s}\xspace}
\def\Dsb     {\ensuremath{\Dbar^+_s}\xspace}
\def\Dss     {\ensuremath{D^{*+}_s}\xspace}


\def\B       {\ensuremath{B}\xspace}
%%% do NOT use ensuremath here
\def\Bbar    {\kern 0.18em\overline{\kern -0.18em B}{}\xspace}
\def\Bb      {\ensuremath{\Bbar}\xspace}
\def\BB      {\ensuremath{B\Bbar}\xspace} 
\def\Bz      {\ensuremath{B^0}\xspace}
\def\Bzb     {\ensuremath{\Bbar^0}\xspace}
\def\BzBzb   {\ensuremath{\Bz {\kern -0.16em \Bzb}}\xspace}
\def\Bu      {\ensuremath{B^+}\xspace}
\def\Bub     {\ensuremath{B^-}\xspace}
\def\Bp      {\ensuremath{\Bu}\xspace}
\def\Bm      {\ensuremath{\Bub}\xspace}
\def\Bpm     {\ensuremath{B^\pm}\xspace}
\def\Bmp     {\ensuremath{B^\mp}\xspace}
\def\BpBm    {\ensuremath{\Bu {\kern -0.16em \Bub}}\xspace}
\def\Bs      {\ensuremath{B_s}\xspace}
\def\Bsb     {\ensuremath{\Bbar_s}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%% ONIA %%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\jpsi     {\ensuremath{{J\mskip -3mu/\mskip -2mu\psi\mskip 2mu}}\xspace}
\def\psitwos  {\ensuremath{\psi{(2S)}}\xspace}
\def\psiprpr  {\ensuremath{\psi(3770)}\xspace}
\def\etac     {\ensuremath{\eta_c}\xspace}
\def\chiczero {\ensuremath{\chi_{c0}}\xspace}
\def\chicone  {\ensuremath{\chi_{c1}}\xspace}
\def\chictwo  {\ensuremath{\chi_{c2}}\xspace}
\mathchardef\Upsilon="7107
\def\Y#1S{\ensuremath{\Upsilon{(#1S)}}\xspace}% no space before {...}!
\def\OneS  {\Y1S}
\def\TwoS  {\Y2S}
\def\ThreeS{\Y3S}
\def\FourS {\Y4S}
\def\FiveS {\Y5S}
\def\SixS  {\Y6S}

\def\chic#1{\ensuremath{\chi_{c#1}}\xspace} 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%% BARYONS %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\proton      {\ensuremath{p}\xspace}
\def\antiproton  {\ensuremath{\overline p}\xspace}
\def\neutron     {\ensuremath{n}\xspace}
\def\antineutron {\ensuremath{\overline n}\xspace}

\mathchardef\Deltares="7101
\mathchardef\Xi="7104
\mathchardef\Lambda="7103
\mathchardef\Sigma="7106
\mathchardef\Omega="710A

%%% do NOT use ensuremath here
\def\Deltabar{\kern 0.25em\overline{\kern -0.25em \Deltares}{}\xspace}
\def\Lbar{\kern 0.2em\overline{\kern -0.2em\Lambda\kern 0.05em}\kern-0.05em{}\xspace}
\def\Sigbar{\kern 0.2em\overline{\kern -0.2em \Sigma}{}\xspace}
\def\Xibar{\kern 0.2em\overline{\kern -0.2em \Xi}{}\xspace}
\def\Obar{\kern 0.2em\overline{\kern -0.2em \Omega}{}\xspace}
\def\Nbar{\kern 0.2em\overline{\kern -0.2em N}{}\xspace}
\def\Xb{\kern 0.2em\overline{\kern -0.2em X}{}\xspace}

\def\X {\ensuremath{X}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% ENERGY AND MOMENTUM %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\tev}{\ensuremath{\mathrm{\,Te\kern -0.1em V}}\xspace}
\newcommand{\gev}{\ensuremath{\mathrm{\,Ge\kern -0.1em V}}\xspace}
\newcommand{\mev}{\ensuremath{\mathrm{\,Me\kern -0.1em V}}\xspace}
\newcommand{\kev}{\ensuremath{\mathrm{\,ke\kern -0.1em V}}\xspace}
\newcommand{\ev}{\ensuremath{\mathrm{\,e\kern -0.1em V}}\xspace}
\newcommand{\gevc}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V\!/}c}}\xspace}
\newcommand{\mevc}{\ensuremath{{\mathrm{\,Me\kern -0.1em V\!/}c}}\xspace}
\newcommand{\gevcc}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V\!/}c^2}}\xspace}
\newcommand{\mevcc}{\ensuremath{{\mathrm{\,Me\kern -0.1em V\!/}c^2}}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% DISTANCE AND AREA %%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\syin {\ensuremath{^{\prime\prime}}\xspace}
\def\inch   {\ensuremath{\rm \,in}\xspace} % \in is taken
\def\ft   {\ensuremath{\rm \,ft}\xspace}
\def\km   {\ensuremath{{\rm \,km}}\xspace}
\def\m    {\ensuremath{{\rm \,m}}\xspace}
\def\cm   {\ensuremath{{\rm \,cm}}\xspace}
\def\cma  {\ensuremath{{\rm \,cm}^2}\xspace}
\def\mm   {\ensuremath{{\rm \,mm}}\xspace}
\def\mma  {\ensuremath{{\rm \,mm}^2}\xspace}
\def\mum  {\ensuremath{{\,\mu\rm m}}\xspace}%% mu meter 
\def\muma       {\ensuremath{{\,\mu\rm m}^2}\xspace}
\def\nm   {\ensuremath{{\rm \,nm}}\xspace}
\def\fm   {\ensuremath{{\rm \,fm}}\xspace}
\def\nm         {\ensuremath{{\rm \,nm}}\xspace}   %% nanometer
%
\def\barn{\ensuremath{{\rm \,b}}\xspace}
\def\barnhyph{\ensuremath{{\rm -b}}\xspace}
\def\mbarn{\ensuremath{{\rm \,mb}}\xspace}
\def\mbarnhyph{\ensuremath{{\rm -mb}}\xspace}
\def\nb         {\ensuremath{{\rm \,nb}}\xspace}
\def\invnb {\ensuremath{\mbox{\,nb}^{-1}}\xspace}
\def\pb {\ensuremath{{\rm \,pb}}\xspace}
\def\invpb {\ensuremath{\mbox{\,pb}^{-1}}\xspace}
\def\fb   {\ensuremath{\mbox{\,fb}}\xspace}
\def\invfb   {\ensuremath{\mbox{\,fb}^{-1}}\xspace}
\def\invab   {\ensuremath{\mbox{\,ab}^{-1}}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% TIME AND MASS  %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\mus  {\ensuremath{\rm \,\mus}\xspace}
\def\ns   {\ensuremath{\rm \,ns}\xspace}
\def\ps   {\ensuremath{\rm \,ps}\xspace}
\def\fs   {\ensuremath{\rm \,fs}\xspace}
\def\gm   {\ensuremath{\rm \,g}\xspace}

\def\sec{\ensuremath{\rm {\,s}}\xspace}       %% second 
\def\ms         {\ensuremath{{\rm \,ms}}\xspace}     %% millisecond
\def\mus        {\ensuremath{\,\mu{\rm s}}\xspace}    %% microsecond
\def\ns         {\ensuremath{{\rm \,ns}}\xspace}      %% nanosecond
\def\ps         {\ensuremath{{\rm \,ps}}\xspace}  %% picosecond


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%   MISCELLANEOUS %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\Xrad {\ensuremath{X_0}\xspace}
\def\NIL{\ensuremath{\lambda_{int}}\xspace}
\let\dgr\degrees

\def\cms         {\ensuremath{{\rm \,cm}^{-2} {\rm s}^{-1}}\xspace}

\def\mic  {\ensuremath{\,\mu{\rm C}}\xspace}
\def\krad {\ensuremath{\rm \,krad}\xspace}
\def\cmc  {\ensuremath{{\rm \,cm}^3}\xspace}
\def\yr   {\ensuremath{\rm \,yr}\xspace}
\def\hr   {\ensuremath{\rm \,hr}\xspace}
\def\degc {\ensuremath{^\circ}{C}\xspace}
\def\degk {\ensuremath {\rm K}\xspace}
\def\degrees{\ensuremath{^{\circ}}\xspace}
\def\mrad{\ensuremath{\rm \,mrad}\xspace}               %% milliradian
\def\rad{\ensuremath{\rm \,rad}\xspace}
\def\mradhyph{\ensuremath{\rm -mr}\xspace}
%
\def\sx    {\ensuremath{\sigma_x}\xspace}    
\def\sy    {\ensuremath{\sigma_y}\xspace}   
\def\sz    {\ensuremath{\sigma_z}\xspace}    


\def\order{{\ensuremath{\cal O}}\xspace}
\def\L{{\ensuremath{\cal L}}\xspace}
\def\calL{{\ensuremath{\cal L}}\xspace}
\def\calS{{\ensuremath{\cal S}}\xspace}
\def\calA{{\ensuremath{\cal A}}\xspace}
\def\calD{{\ensuremath{\cal D}}\xspace}
\def\calR{{\ensuremath{\cal R}}\xspace}

%% Arrows:
\def\ra                 {\ensuremath{\rightarrow}\xspace}
\def\to                 {\ensuremath{\rightarrow}\xspace}


%%%%%%%%%%%%%%%
%% definitions by Tayduganov
%%%%%%%%%%%%%%%
\def\M{\mathcal{M}}
\def\A{\mathcal{A}}
\def\Op{\mathcal{O}^{\,\prime}}
\def\OOp{\mathcal{O}^{\,(\prime)}}
\def\Cp{C^{\,\prime}}


\newcommand{\stat}{\ensuremath{\mathrm{(stat)}}\xspace}
\newcommand{\syst}{\ensuremath{\mathrm{(syst)}}\xspace}

\newcommand{\inverse}{\ensuremath{^{-1}}\xspace}
\newcommand{\dedx}{\ensuremath{\mathrm{d}\hspace{-0.1em}E/\mathrm{d}x}\xspace}
\newcommand{\chisq}{\ensuremath{\chi^2}\xspace}
\newcommand{\delm}{\ensuremath{m_{\dstr}-m_{\dz}}\xspace}
\newcommand{\lum} {\ensuremath{\mathcal{L}}\xspace}

\def\gsim{{~\raise.15em\hbox{$>$}\kern-.85em
          \lower.35em\hbox{$\sim$}~}\xspace}
\def\lsim{{~\raise.15em\hbox{$<$}\kern-.85em
          \lower.35em\hbox{$\sim$}~}\xspace}

\def\qsq                {\ensuremath{q^2}\xspace}

%%%%% macros used in theory chapters (Theory, WG9...)
\newcommand{\ov}{\overline}
\newcommand{\Lag}{\ensuremath{\mathcal{L}}}
% Quarks and gluons
%
\newcommand{\qq}{\ensuremath{q}\xspace}
\newcommand{\uq}{\ensuremath{u}\xspace}
\newcommand{\dq}{\ensuremath{d}\xspace}
\newcommand{\sq}{\ensuremath{s}\xspace}
\newcommand{\cq}{\ensuremath{c}\xspace}
\newcommand{\bq}{\ensuremath{b}\xspace}
\newcommand{\tq}{\ensuremath{t}\xspace}
% \newcommand{\qbar}{\ensuremath{\bar{q}}\xspace}
\newcommand{\qbarq} {\ensuremath{q\bar{q}}\xspace} 
%
\newcommand{\ubarq}{\ensuremath{\bar{u}}\xspace}
\newcommand{\dbarq}{\ensuremath{\bar{d}}\xspace}
\newcommand{\sbarq}{\ensuremath{\bar{s}}\xspace}
\newcommand{\cbarq}{\ensuremath{\bar{c}}\xspace}
\newcommand{\bbarq}{\ensuremath{\bar{b}}\xspace}
\newcommand{\tbarq}{\ensuremath{\bar{t}}\xspace}
\newcommand{\lt}{\left}
\newcommand{\rt}{\right}
%\newcommand{\gev}{\,\mbox{GeV}}
%\newcommand{\tev}{\,\mbox{TeV}}
%\newcommand{\mev}{\,\mbox{MeV}}
\newcommand{\eq}[1]{Eq.~(\ref{#1})}
\newcommand{\eqsand}[2]{Eqs.~(\ref{#1}) and (\ref{#2})}
\newcommand{\eqsto}[2]{Eqs.~(\ref{#1}--\ref{#2})}
\newcommand{\ds}{\displaystyle}
\newcommand{\PARITY}{\ensuremath{P}\xspace}
\newcommand{\CCC}{\ensuremath{C}\xspace}
\newcommand{\TTT}{\ensuremath{T}\xspace}
\newcommand{\CP}{\ensuremath{CP}\xspace}
\newcommand{\CPT}{\ensuremath{CPT}\xspace}
\newcommand{\Wb}{\ensuremath{W}\xspace}
\newcommand{\Zb}{\ensuremath{Z}\xspace}
\newcommand{\im}{\mathrm{Im}\xspace}
\newcommand{\real}{\mathrm{Re}\xspace}
\newcommand{\Bodbar}{\ensuremath{\overline{B}{}^{0}_{d}}\xspace}
\newcommand{\bbd}{\ensuremath{B^0_d\!-\!\overline{B}{}^0_d}\,}
\newcommand{\bbmd}{\bbd\ mixing\xspace}
\newcommand{\alpS}{\ensuremath{\alpha_{s}}\xspace}
\newcommand{\LambdaQCD}{\ensuremath{\Lambda_{\text{QCD}}}\xspace}
\newcommand{\MW}{\ensuremath{M_{W}}\xspace}
\newcommand{\GF}{\ensuremath{G_{\text{F}}}\xspace}
\newcommand{\Vqd}{\ensuremath{V_{qd}}\xspace}
\newcommand{\Vqs}{\ensuremath{V_{qs}}\xspace}
\newcommand{\Vqb}{\ensuremath{V_{qb}}\xspace}
\newcommand{\Vud}{\ensuremath{V_{ud}}\xspace}
\newcommand{\Vus}{\ensuremath{V_{us}}\xspace}
\newcommand{\Vub}{\ensuremath{V_{ub}}\xspace}
\newcommand{\Vcd}{\ensuremath{V_{cd}}\xspace}
\newcommand{\Vcq}{\ensuremath{V_{cq}}\xspace}
\newcommand{\Vuq}{\ensuremath{V_{uq}}\xspace}
\newcommand{\Vcs}{\ensuremath{V_{cs}}\xspace}
\newcommand{\Vcb}{\ensuremath{V_{cb}}\xspace}
\newcommand{\Vtd}{\ensuremath{V_{td}}\xspace}
\newcommand{\Vts}{\ensuremath{V_{ts}}\xspace}
\newcommand{\Vtb}{\ensuremath{V_{tb}}\xspace}
\newcommand{\Vtq}{\ensuremath{V_{tq}}\xspace}
\newcommand{\ket}[1]{\ensuremath{\big|{#1}\big\rangle}}
\newcommand{\bra}[1]{\ensuremath{\big\langle{#1}\big|}}
\newcommand{\brax}[1]{\ensuremath{\big\langle{#1}}}   % No ``|''
\newcommand{\braket}[2]{\brax{#1}\ket{#2}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%TDCPV  WG3
\def\permille{\ensuremath{{}^\text{o}\mkern-5mu/\mkern-3mu_\text{oo}}}
\renewcommand{\sectionmark}[1]{\markright{\thesection\ #1}}

%%%%%
%% WG6

\def\DstpDzPip{$D^{*+}\rightarrow D^0\pi^+$}
\def\DzKPi{$D^0\rightarrow K\pi$}
\def\DzKK{$D^0\rightarrow \Kp\Km$}
\def\sigmat{$\sigma_t$}
\def\babar{BaBar}
\def\deltam{$\Delta m$}
\def\dWS {D^{0}\to\Kp\pim\piz}
\def\dRS {D^{0}\to\Km\pip\piz}
\def\BES {\text{BES{\ }\uppercase\expandafter{\romannumeral3}}}
\def\BTWO {\text{Belle{\ }\uppercase\expandafter{\romannumeral2}}}
\def\disc {\textcolor{red}{$\bigstar$}}
%\def\evid {\textcolor{red}{$\ding{73}$}}
\def\evid {\textcolor{green}{$\bullet$}}
\def\meas {\textcolor{blue}{$\checkmark$}}
%\DeclareMathOperator\RE{Re}
%\DeclareMathOperator\IM{Im}
\def\ccss{\ensuremath{c\overline c s \overline s}\xspace}
\def\outbdt {\ensuremath{\text{Out}_{\text{FBDT}}}\xspace}
\newcommand{\splot}{\hbox{$_s$}{\cal P}lot}


%%%%%%%%%%%%
%% WG8
\newcommand{\bit}[1]{\boldsymbol{\mathcal{#1}}}
\newcommand{\der}{\stackrel{\leftrightarrow}{D}}
\newcommand{\derleft}{\stackrel{\leftarrow}{D}}
\newcommand{\derright}{\stackrel{\rightarrow}{D}}
\newcommand{\sder}{\not\stackrel{\leftrightarrow}{D}}
\newcommand{\sderleft}{\not\stackrel{\leftarrow}{D}}
\newcommand{\sderright}{\not\stackrel{\rightarrow}{D}}
\newcommand{\psibar}{{\bar{\psi}}}
\newcommand{\re}{\hbox{Re}}
\newcommand{\mpid}{m^2_{\pi}}
\newcommand{\mkd}{m^2_K}

%%%%%%%%%%%%%%
%% svd paper SOFTWARE chapter
\newcommand{\nc}[1]{\texttt{#1}}
\newcommand{\ioct}[1]{\texttt{#1}}
\def\basf{\textit{basf2}}
%\newcommand{\snr}{\ensuremath{\mathrm{S}\hspace{-0.1em}\mathrm{N}\hspace{-0.1em}\mathrm{R}}\xspace}
\newcommand{\snr}{\ensuremath{\mathrm{SNR}}\xspace}
\newcommand{\snrST}{\ensuremath{\snr_\mathrm{strip}}\xspace}
\newcommand{\snrZS}{\ensuremath{\snr_\mathrm{ZS}}\xspace}
\newcommand{\snrADJ}{\ensuremath{\snr_\mathrm{adj}}\xspace}
\newcommand{\snrSEED}{\ensuremath{\snr_\mathrm{seed}}\xspace}
\newcommand{\snrCL}{\snr}
%\newcommand{\snrCL}{\ensuremath{\snr_\mathrm{CL}}\xspace}
\def\uP{u/P\xspace}
\def\vN{v/N\xspace}
\def\traw{\ensuremath{t_{\rm raw}}}
\def\thit{\ensuremath{t_{\rm hit}}}
\def\tZ{\ensuremath{t_0}}
\def\eventtz{event $t_0$}
\def\tZsvd{\ensuremath{t_0^{\rm svdRF}}}
% Tsuboyama 


\usepackage{textgreek}

%\newcommand{\mul}{$\times$}
% \newcommand{\mum}{$\rm{\mu}$m}
%\newcommand{\ohm}{$\rm{\Omega}$}
%\newcommand{\PM}{$\pm$}
% \newcommand{\DEG}{$^\circ$}  use \degrees
%\newcommand{\COtwo}{CO$_2$\ }

\newcommand{\mul}{$\times$}
\newcommand{\um}{\textmu m}
\newcommand{\us}{\textmu s}
% \newcommand{\ohm}{\textOmega}
\newcommand{\PM}{$\pm$}
%\newcommand{\DEG}{$^\circ$}
%\newcommand{\etal}{\textit{et al}.}
\newcommand{\SR}{$^{90}$Sr}

